Two-Grid Methods for Semilinear Interface Problems

In this article we consider two-grid finite element methods for solving semilinear interface problems in d space dimensions, for d=2 or d=3. We first describe in some detail the target problem class with discontinuous diffusion coefficients, which includes problems containing sub-critical, critical, and supercritical nonlinearities. We then establish basic quasi-optimal a priori error estimate for Galerkin approximations. In the critical and subcritical cases, we follow our recent approach to controling the nonlinearity using only pointwise control of the continuous solution and a local Lipschitz property, rather than through pointwise control of the discrete solution; this eliminates the requirement that the discrete solution satisfy a discrete form of the maximum principle, hence eliminating the need for restrictive angle conditions in the underlying mesh. The supercritical case continues to require such mesh conditions in order to control the nonlinearity. We then design a two-grid algorithm consisting of a coarse grid solver for the original nonlinear problem, and a fine grid solver for a linearized problem. We analyze the quality of approximations generated by the algorithm, and show that the coarse grid may be taken to have much larger elements than the fine grid, and yet one can still obtain approximation quality that is asymptotically as good as solving the original nonlinear problem on the fine mesh. The algorithm we describe, and its analysis in this article, combines four sets of tools: the work of Xu and Zhou on two-grid algorithms for semilinear problems; the recent results for linear interface problems due to Li, Melenk, Wohlmuth, and Zou; recent work on the Poisson-Boltzmann equation; and recent work on a priori estimates for semilinear problems.

==> app.tex <==
\appendix
\addtocontents{toc}{\protect\setcounter{tocdepth}{1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some Supporting Results}
\label{app:entire}

In this appendix we assemble some supporting results that we
exploit at various points in the body of the paper.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Some Comments}

For the nonlinear interface problem, we usually do not have this nice regularity.
So the main task of the remainder of this section is to discuss the estimate of $\tbar u - u_{h} \tbar$ and $\|u-u_{h}\|_{0,4}$ for the interface problem.


For the $L^4$ estimate, we can use one of two approaches.
The first approach is a general inequality based on norm-comparability at the discrete level.
The second approach uses the Ladyzhenskaya inequality
$$ \| u \|_{0,4} \le \left(\frac{4}{3}\right)^{\frac{3}{8}}\|u\|_{0,2}^{\frac{1}{4}} \| \nabla u\|_{0,2}^{\frac{3}{4}} $$
which holds for any function $u \in W^{1,2}_{0}(\Omega)$ with $\Omega \subset \R^3$.

The norm-comparability approach is as follows.
Let $v \in V_{h}$ be arbitrary.
Using the triangle inequality, we have
$$ \| u - u_{h} \|_{0,4} \le \| u - v \|_{0,4} + \| v - u_{h} \|_{0,4} $$
We handle the second term using norm equivalence in the discrete space, yielding
$$ \| u - u_{h} \|_{0,4} \le \| u - v \|_{0,4} + h^{\sigma} \| v - u_{h} \|_{0,2} $$
where $\sigma$ is WHAT.
We again employ the triengle inequality to arrive at
$$ \| u - u_{h} \|_{0,4} \le \| u - v \|_{0,4} + h^{\sigma} \| u - u_{h} \|_{0,2} + h^{\sigma} \| u - v \|_{0,2}. $$
We may now choose $v$ to be some form of interpolant to arrive at an \emph{a priori} result.

The approach based on the Ladyzhenskaya inequality is much easier.
\mnote{Restructure this to have an overview of the results from Li, et al come before all of these estimates, since it fits into all of these approaches.}

For the energy norm estimate, we will use a quasi-interpolation operator from Li, Melenk, Wohlmuth, and Zou \cite{Li.J;Melenk.J;Wohlmuth.B;Zou.J2010}.
We recall the following quasi-optimal \emph{a priori} estimate.
The Galerkin solution $u_{h} \in V_{h}$ satisfies the following inequality
$$ \tbar u - u_{h} \tbar \le C \inf_{v \in V_{h}} \tbar u - v \tbar $$
where $C$ depends on the PDE, domain, and mesh angles, but not the mesh size.
We can now choose $v = Q_h u$ where $Q_h$ is the quasi-interpolant of Li, et al, which yields the necessary estimates.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{General Discussion Notes}
%
%Let $\tbar v\tbar := \sqrt{a(v,v)}$ be the natural energy norm. It is obvious that $\tbar v\tbar \simeq \|v\|_{1,\Omega}.$ We make the following assumptions on $f$ and the solution $u$
%\begin{enumerate}
%	\item[(A1)] $f$ is a polynomial of degree $m$ with $1\le m <\infty$ when $d =2,$ and $1\le m \le 5$ when $d=3$.
%	\item[(A2)] $u\in H^{1}_{0}(\Omega) \cap H^{s}(\Omega_{1}\cup \Omega_{2})$ for some $s\in (1,2]$. When $d=3,$ we assume $s\in (3/2, 2].$
%	\item[(A3)] $\tbar u - u_{h}\tbar \le M$ for some constant $M>0.$
%\end{enumerate}
%Obviously, assumption (A2) implies that $u\in L^{\infty}(\Omega).$ Also, the assumption (A3) is quite natural from the minimization point of view. 
%

